Study of $b\bar{b}$ correlations in high energy proton-proton collisions

Kinematic correlations for pairs of beauty hadrons, produced in high energy proton-proton collisions, are studied. The data sample used was collected with the LHCb experiment at centre-of-mass energies of 7 and 8 TeV and corresponds to an integrated luminosity of 3 fb$^{-1}$. The measurement is performed using inclusive $b\rightarrow J/\psi X$ decays in the rapidity range $2<y^{J/\psi}<4.5$. The observed correlations are in good agreement with theoretical predictions.

==> LHCb_Authorship_flat_arXiv_06-Jun-2017.tex <==
LHCb collaboration: 
R. Aaij,
B. Adeva,
M. Adinolfi,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
S. Ali,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
S. Amerio,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
M. Andreotti,
J.E. Andrews,
R.B. Appleby,
F. Archilli,
P. d'Argent,
J. Arnau Romeu,
A. Artamonov,
M. Artuso,
E. Aslanides,
G. Auriemma,
M. Baalouch,
I. Babuschkin,
S. Bachmann,
J.J. Back,
A. Badalov,
C. Baesso,
S. Baker,
V. Balagura,
W. Baldini,
A. Baranov,
R.J. Barlow,
C. Barschel,
S. Barsuk,
W. Barter,
F. Baryshnikov,
V. Batozskaya,
V. Battista,
A. Bay,
L. Beaucourt,
J. Beddow,
F. Bedeschi,
I. Bediaga,
A. Beiter,
L.J. Bel,
N. Beliy,
V. Bellee,
N. Belloli,
K. Belous,
I. Belyaev,
E. Ben-Haim,
G. Bencivenni,
S. Benson,
S. Beranek,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.-O. Bettler,
M. van Beuzekom,
Ia. Bezshyiko,
S. Bifani,
P. Billoir,
A. Birnkraut,
A. Bitadze,
A. Bizzeti,
M. Bj{\o}rn,
T. Blake,
F. Blanc,
J. Blouw,
S. Blusk,
V. Bocci,
T. Boettcher,
A. Bondar,
N. Bondar,
W. Bonivento,
I. Bordyuzhin,
A. Borgheresi,
S. Borghi,
M. Borisyak,
M. Borsato,
F. Bossu,
M. Boubdir,
T.J.V. Bowcock,
E. Bowen,
C. Bozzi,
S. Braun,
T. Britton,
J. Brodzicka,
D. Brundu,
E. Buchanan,
C. Burr,
A. Bursche,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
A. Camboni,
P. Campana,
D.H. Campora Perez,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
P. Carniti,
L. Carson,
K. Carvalho Akiba,
G. Casse,
L. Cassina,
L. Castillo Garcia,
M. Cattaneo,
G. Cavallero,
R. Cenci,
D. Chamont,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
M. Chefdeville,
S. Chen,
S.F. Cheung,
S.-G. Chitic,
V. Chobanova,
M. Chrzaszcz,
A. Chubykin,
P. Ciambrone,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J. Cogan,
E. Cogneras,
V. Cogoni,
L. Cojocariu,
P. Collins,
T. Colombo,
A. Comerma-Montells,
A. Contu,
A. Cook,
G. Coombs,
S. Coquereau,
G. Corti,
M. Corvo,
C.M. Costa Sobral,
B. Couturier,
G.A. Cowan,
D.C. Craik,
A. Crocombe,
M. Cruz Torres,
R. Currie,
C. D'Ambrosio,
F. Da Cunha Marinho,
E. Dall'Occo,
J. Dalseno,
A. Davis,
O. De Aguiar Francisco,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
P. De Simone,
C.T. Dean,
D. Decamp,
L. Del Buono,
H.-P. Dembinski,
M. Demmer,
A. Dendek,
D. Derkach,
O. Deschamps,
F. Dettori,
B. Dey,
A. Di Canto,
P. Di Nezza,
H. Dijkstra,
F. Dordei,
M. Dorigo,
A. Dosil Su{\'a}rez,
L. Douglas,
A. Dovbnya,
K. Dreimanis,
L. Dufour,
G. Dujany,
P. Durante,
R. Dzhelyadin,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
M. Ebert,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
U. Eitschberger,
R. Ekelhof,
L. Eklund,
S. Ely,
S. Esen,
H.M. Evans,
T. Evans,
A. Falabella,
N. Farley,
S. Farry,
R. Fay,
D. Fazzini,
L. Federici,
D. Ferguson,
G. Fernandez,
P. Fernandez Declara,
A. Fernandez Prieto,
F. Ferrari,
F. Ferreira Rodrigues,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiore,
M. Fiorini,
M. Firlej,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
K. Fohl,
M. Fontana,
F. Fontanelli,
D.C. Forshaw,
R. Forty,
V. Franco Lima,
M. Frank,
C. Frei,
J. Fu,
W. Funk,
E. Furfaro,
C. F{\"a}rber,
E. Gabriel,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
M. Gandelman,
P. Gandini,
Y. Gao,
L.M. Garcia Martin,
J. Garc{\'\i}a Pardi{\~n}as,
J. Garra Tico,
L. Garrido,
P.J. Garsed,
D. Gascon,
C. Gaspar,
L. Gavardi,
G. Gazzoni,
D. Gerick,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
Ph. Ghez,
S. Gian{\`\i},
V. Gibson,
O.G. Girard,
L. Giubega,
K. Gizdov,
V.V. Gligorov,
D. Golubkov,
A. Golutvin,
A. Gomes,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
R. Greim,
P. Griffith,
L. Grillo,
L. Gruber,
B.R. Gruberg Cazon,
O. Gr{\"u}nberg,
E. Gushchin,
Yu. Guz,
T. Gys,
C. G{\"o}bel,
T. Hadavizadeh,
C. Hadjivasiliou,
G. Haefeli,
C. Haen,
S.C. Haines,
B. Hamilton,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
S.T. Harnew,
J. Harrison,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heinicke,
A. Heister,
K. Hennessy,
P. Henrard,
L. Henry,
E. van Herwijnen,
M. He{\ss},
A. Hicheur,
D. Hill,
C. Hombach,
P.H. Hopchev,
Z.C. Huard,
W. Hulsbergen,
T. Humair,
M. Hushchyn,
D. Hutchcroft,
P. Ibis,
M. Idzik,
P. Ilten,
R. Jacobsson,
J. Jalocha,
E. Jans,
A. Jawahery,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
C. Joram,
B. Jost,
N. Jurik,
S. Kandybei,
M. Karacson,
J.M. Kariuki,
S. Karodia,
N. Kazeev,
M. Kecke,
M. Kelsey,
M. Kenzie,
T. Ketel,
E. Khairullin,
B. Khanji,
C. Khurewathanakul,
T. Kirn,
S. Klaver,
K. Klimaszewski,
T. Klimkovich,
S. Koliiev,
M. Kolpin,
I. Komarov,
R. Kopecna,
P. Koppenburg,
A. Kosmyntseva,
S. Kotriakhova,
M. Kozeiha,
L. Kravchuk,
M. Kreps,
P. Krokovny,
F. Kruse,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
A.K. Kuonen,
K. Kurek,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
G. Lanfranchi,
C. Langenbruch,
T. Latham,
C. Lazzeroni,
R. Le Gac,
A. Leflat,
J. Lefran{\c{c}}ois,
R. Lef{\`e}vre,
F. Lemaitre,
E. Lemos Cid,
O. Leroy,
T. Lesiak,
B. Leverington,
P.-R. Li,
T. Li,
Y. Li,
Z. Li,
T. Likhomanenko,
R. Lindner,
F. Lionetto,
V. Lisovskyi,
X. Liu,
D. Loh,
A. Loi,
I. Longstaff,
J.H. Lopes,
D. Lucchesi,
A. Luchinsky,
M. Lucio Martinez,
H. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Maev,
K. Maguire,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
A. Malinin,
T. Maltsev,
G. Manca,
G. Mancinelli,
P. Manning,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
G. Martellotti,
M. Martin,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
D. Martins Tostes,
L.M. Massacrier,
A. Massafferri,
R. Matev,
A. Mathad,
Z. Mathe,
C. Matteuzzi,
A. Mauri,
E. Maurice,
B. Maurin,
A. Mazurov,
M. McCann,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
F. Meier,
N. Meinert,
D. Melnychuk,
M. Merk,
A. Merli,
E. Michielin,
D.A. Milanes,
E. Millard,
M.-N. Minard,
L. Minzoni,
D.S. Mitzel,
A. Mogini,
J. Molina Rodriguez,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
M.J. Morello,
O. Morgunova,
J. Moron,
A.B. Morris,
R. Mountain,
F. Muheim,
M. Mulder,
D. M{\"u}ller,
J. M{\"u}ller,
K. M{\"u}ller,
V. M{\"u}ller,
P. Naik,
T. Nakada,
R. Nandakumar,
A. Nandi,
I. Nasteva,
M. Needham,
N. Neri,
S. Neubert,
N. Neufeld,
M. Neuner,
T.D. Nguyen,
C. Nguyen-Mau,
S. Nieswand,
R. Niet,
N. Nikitin,
T. Nikodem,
A. Nogay,
D.P. O'Hanlon,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
R. Oldeman,
C.J.G. Onderwater,
A. Ossowska,
J.M. Otalora Goicochea,
P. Owen,
A. Oyanguren,
P.R. Pais,
A. Palano,
M. Palutan,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
W. Parker,
C. Parkes,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
A. Pearce,
A. Pellegrino,
G. Penso,
M. Pepe Altarelli,
S. Perazzini,
P. Perret,
L. Pescatore,
K. Petridis,
A. Petrolini,
A. Petrov,
M. Petruzzo,
E. Picatoste Olloqui,
B. Pietrzyk,
M. Pikies,
D. Pinci,
F. Pisani,
A. Pistone,
A. Piucci,
V. Placinta,
S. Playfer,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
A. Poluektov,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Poslavskii,
C. Potterat,
E. Price,
J. Prisciandaro,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
R. Quagliani,
B. Quintana,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
I. Raniuk,
F. Ratnikov,
G. Raven,
M. Ravonel Salzgeber,
M. Reboud,
F. Redi,
S. Reichert,
A.C. dos Reis,
C. Remon Alepuz,
V. Renaudin,
S. Ricciardi,
S. Richards,
M. Rihl,
K. Rinnert,
V. Rives Molina,
P. Robbe,
A. Robert,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
P. Rodriguez Perez,
A. Rogozhnikov,
S. Roiser,
A. Rollings,
V. Romanovskiy,
A. Romero Vidal,
J.W. Ronayne,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
P. Ruiz Valls,
J. Ruiz Vidal,
J.J. Saborido Silva,
E. Sadykhov,
N. Sagidova,
B. Saitta,
V. Salustino Guimaraes,
C. Sanchez Mayordomo,
B. Sanmartin Sedes,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
G. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
D.M. Saunders,
D. Savrina,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schlupp,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
H.F. Schreiner,
K. Schubert,
M. Schubiger,
M.-H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
A. Semennikov,
E.S. Sepulveda,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
P. Seyfert,
M. Shapkin,
I. Shapoval,
Y. Shcheglov,
T. Shears,
L. Shekhtman,
V. Shevchenko,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
M. Sirendi,
N. Skidmore,
T. Skwarnicki,
E. Smith,
I.T. Smith,
J. Smith,
M. Smith,
l. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
B. Souza De Paula,
B. Spaan,
P. Spradlin,
S. Sridharan,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
S. Stefkova,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
M. Stepanova,
H. Stevens,
S. Stone,
B. Storaci,
S. Stracka,
M.E. Stramaglia,
M. Straticiuc,
U. Straumann,
L. Sun,
W. Sutcliffe,
K. Swientek,
V. Syropoulos,
M. Szczekowski,
T. Szumlak,
M. Szymanski,
S. T'Jampens,
A. Tayduganov,
T. Tekampe,
G. Tellarini,
F. Teubert,
E. Thomas,
J. van Tilburg,
M.J. Tilley,
V. Tisserand,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Tonelli,
F. Toriello,
R. Tourinho Jadallah Aoude,
E. Tournefier,
M. Traill,
M.T. Tran,
M. Tresch,
A. Trisovic,
A. Tsaregorodtsev,
P. Tsopelas,
A. Tully,
N. Tuning,
A. Ukleja,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
C. Vacca,
A. Vagner,
V. Vagnoni,
A. Valassi,
S. Valat,
G. Valenti,
R. Vazquez Gomez,
P. Vazquez Regueiro,
S. Vecchi,
M. van Veghel,
J.J. Velthuis,
M. Veltri,
G. Veneziano,
A. Venkateswaran,
T.A. Verlage,
M. Vernet,
M. Vesterinen,
J.V. Viana Barbosa,
B. Viaud,
D.  Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
M. Vitti,
V. Volkov,
A. Vollhardt,
B. Voneki,
A. Vorobyev,
V. Vorobyev,
C. Vo{\ss},
J.A. de Vries,
C. V{\'a}zquez Sierra,
R. Waldi,
C. Wallace,
R. Wallace,
J. Walsh,
J. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
D. Websdale,
A. Weiden,
M. Whitehead,
J. Wicht,
G. Wilkinson,
M. Wilkinson,
M. Williams,
M.P. Williams,
M. Williams,
T. Williams,
F.F. Wilson,
J. Wimberley,
M. Winn,
J. Wishahi,
W. Wislicki,
M. Witek,
G. Wormser,
S.A. Wotton,
K. Wraight,
K. Wyllie,
Y. Xie,
Z. Xu,
Z. Yang,
Z. Yang,
Y. Yao,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
L. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}

